The Approximate Fisher Influence Function: Faster Estimation of Data Influence in Statistical Models

Quantifying the influence of infinitesimal changes in training data on model performance is crucial for understanding and improving machine learning models. In this work, we reformulate this problem as a weighted empirical risk minimization and enhance existing influence function-based methods by using information geometry to derive a new algorithm to estimate influence. Our formulation proves versatile across various applications, and we further demonstrate in simulations how it remains informative even in non-convex cases. Furthermore, we show that our method offers significant computational advantages over current Newton step-based methods.

==> background.tex <==
\subsection{Related work}
% \vspace{-4.5pt}
A common approach to approximating $\hat{\theta}(w^{n})$ is to optimize a surrogate to the loss function $L(\mD, \theta, \lambda, w^{n})$. This paper focuses on methods based on {\em quadratic approximations of the objective} \citep{cook1980characterizations, KohLiang_Influence_DL, giordano2019swiss, Wilson_OptimizerComparison}, which provide computationally efficient estimates while maintaining accuracy. These approximations yield solutions of the form:
\begin{align}
    \tilde{\theta}(w^{n}) = \hat{\theta}(\boldsymbol{1}) - \brC(\hat{\theta}(\boldsymbol{1}), w^{n}) b(\hat{\theta}(\boldsymbol{1}), w^{n}),
\end{align}
where $b(\cdot, \cdot)$ and $\brC(\cdot, \cdot)$ depend on the specific loss approximation and vary across applications.

A notable instance of this framework is the \emph{infinitesimal jackknife} (IJ) approximation, denoted $\tilde{\theta}^{\mathrm{IJ}}(w^n)$, which is defined via a Newton step:
\begin{align}
    \label{eq:G_Definition}
    b(\hat{\theta}(\boldsymbol{1}), w^{n}) &\triangleq \frac{1}{n} \sum_{i=1}^{n} \nabla_{\theta} \ell(z_i, \hat{\theta}(\boldsymbol{1})) (w_i - 1), \\
    \brC(\hat{\theta}(\boldsymbol{1}), \boldsymbol{1}) &= \nabla^{2}_{\theta} L(\mD, \hat{\theta}(\boldsymbol{1}), \boldsymbol {1})^{-1} \triangleq \brH(\hat{\theta}(\boldsymbol{1}), \boldsymbol{1})^{-1}.
\end{align}
Several works have established the accuracy of this approximation under specific conditions on the loss function and the weight vectors $w^{n}$ \citep{giordano2019swiss}. These results hold under subsets of the following assumptions.

\begin{assump}[Curvature of the Objective]
    \label{ass:one_1}
    For each $i \in [n]$, the function $\frac{1}{n} \ell(z_i, \theta)$ is $\mu$-strongly convex ($\mu > 0$), and the prior $\pi(\theta)$ is convex.
\end{assump}  

\begin{assump}[Lipschitz Hessian of the Objective]
    \label{ass:two_1}
    For each $i \in [n]$, the function $\frac{1}{n} \ell(z_i, \theta)$ is twice differentiable with an $M$-Lipschitz Hessian.
\end{assump}

\begin{assump}[Smooth Hessian of the Objective]
    \label{ass:two_11}
    For each $i \in [n]$, the function $\frac{1}{n} \ell(z_i, \theta)$ is twice differentiable with a $C$-smooth Hessian.
\end{assump}

\begin{assump}[Bounded Moments]
    \label{ass:boundedmoments}
    For given $s, r \geq 0$, the quantity $B_{sr}$ is finite, where
    \begin{align}
        B_{sr} \triangleq \frac{1}{n} \sum_{i=1}^n \text{Lip}(\nabla_\theta \ell(z_i, \cdot))^s \|\nabla_{\theta} \ell(z_i, \hat{\theta}(\boldsymbol{1}))\|^{r}.
    \end{align}
\end{assump}

\begin{assump}[Lipschitz Features]
    \label{ass:LipFeatures}
    The feature mapping $f(x_i; \theta)$ is $C_f$-Lipschitz with a $\tilde{C}_f$-Lipschitz gradient for all $i \in [n]$.
\end{assump}

\begin{assump}[Lipschitz Inference Objective]
    \label{ass:Lipschitz_T}
    The inference objective $T(\theta, w^n)$ is twice differentiable, $C_{T_1}$-Lipschitz, and has a $C_{T_2}$-Lipschitz gradient with respect to $\theta$ for $w^n \in \mathcal{D}^{-i}$ and all $i \in [n]$.
\end{assump}

For the examples in \secref{s:ProblemDef}, the following guarantees hold: 

%For the examples in \secref{s:ProblemDef}, the following guarantees were obtained: 
\begin{prop}[LOOCV Approximation Bound~(\cite{Wilson_OptimizerComparison}, Thm.~4)]
    \label{prop:CV_Guarantees_Wilson}
    Suppose \assref{ass:one_1}, \assref{ass:two_1}, and \assref{ass:boundedmoments} hold for $(s,r) = \{(0,3), (1,3), (1,4), (1,2), (2,2), (3,2)\}$. When the infinitesimal jackknife (IJ) is used as a plug-in estimate for the leave-one-out cross-validation (LOOCV) objective, 
    \[
    T_i(\theta) \triangleq T(\theta, w^n) = \frac{1}{n} \ell(z_i, \theta),
    \]
    with $w^n \in \mathcal{D}^{-i}$, the error in this approximation is bounded as
    \begin{align}
        \left| \sum_{i=1}^n \left( T_i(\tilde{\theta}^{\mathrm{IJ}}(w^n)) - T_i(\hat{\theta}(w^n)) \right) \right| = O\left(\frac{M B_{03}}{\mu^3 n^2} + \frac{B_{12}}{\mu^2 n^2} \right).
    \end{align}
\end{prop}
% \begin{prop}[LOOCV~(\cite{Wilson_OptimizerComparison}, Thm.~4)]
% \label{prop:CV_Guarantees_Wilson}  Suppose \assref{ass:one_1}, \ref{ass:two_1} and \ref{ass:boundedmoments} for $(s,r) = \{(0,3), (1,3),(1,4), (1,2), (2,2), (3,2)\}$ holds. When the IJ is used as plug-in estimate to the {\em LOOCV} objective $T_i(\theta)\triangleq T(\theta, \boldsymbol{1}^{n\backslash i})  = \frac{1}{n}\ell(z_i, \theta) $, the error in this approximation can be bounded as, 
% % \vspace{0pt}
% \begin{align}
%     &|\sum_{i=1}^n (T_i(\tilde{\theta}^{\mathrm{IJ}}(\boldsymbol{1}^{n\backslash i})) - T_i(\hat{\theta}(\boldsymbol{1}^{n\backslash i})))| = O(\frac{MB_{03}}{\mu^3 n^2} + \frac{B_{12}}{\mu^2 n^2}).
% \end{align}
% \end{prop}

The next proposition relies on the $(\eps,\delta)$-unlearning definition from \citep{Sekhari_Unlearning_Neurips}.
\begin{prop}[Machine Unlearning~\citep{WilsonSuriyakumar_UnlearningProximal}]
    \label{prop:unlearning_wilson}  
    Suppose $\ell(z, \theta)$ is $\mu$-strongly convex, twice differentiable, $L$-Lipschitz, with a $C$-smooth and $M$-Lipschitz Hessian for all $z$, and that $\pi(\theta)$ is convex.\footnote{These assumptions strengthen \assref{ass:one_1}-\assref{ass:boundedmoments}, requiring Lipschitz continuity for any $z$, not just the training samples $\{z_i\}$.} When the infinitesimal jackknife (IJ) is used as a plug-in estimate for the objective $T(\theta) = \theta$, we have
    \begin{align}
        \| T(\tilde{\theta}^{\mathrm{IJ}}(w^n)) - T(\hat{\theta}(w^n))\| \leq \frac{2ML}{n^2\mu^2} + \frac{CL^2}{n^2\mu^3}, \quad \text{for } w^n \in \mathcal{D}^{-i}.
    \end{align}
    Furthermore, the algorithm returning $\tilde{\theta}^{\mathrm{IJ}}(w^n) + \zeta$ for $w^n \in \mathcal{D}^{-i}$ satisfies $(\eps,\delta)$-unlearning, where $\zeta \sim \mathcal{N}(0, c\brI)$ with $
    c = (2\mu ML + CL^2) \sqrt{2\log(5/4\delta)}/\eps \mu^{3} n^{2}.$ 
\end{prop} 


\begin{prop}[Data Attribution~(\cite{koh2019accuracy}, Prop.~1)]
    \label{prop:attributions}
    Suppose \assref{ass:one_1}, \assref{ass:two_1}, and \assref{ass:Lipschitz_T} hold, and that $\pi(\theta) = \norm{\theta}^2$. Define $C_{\ell} \triangleq \max_{i\in[n]} \|\nabla \ell(z_i, \hat{\theta}(\boldsymbol{1}))\|$. When the infinitesimal jackknife (IJ) is used as a plug-in estimate for the inference objective 
    \[
    T(\theta) = \ell(z_{\mathrm{test}}, \theta) - \ell(z_{\mathrm{test}}, \hat\theta(\boldsymbol{1})),
    \]
    the approximation error is bounded as
    \begin{align}
        \left|T(\hat{\theta}(w^n)) - T(\tilde{\theta}^{\mathrm{IJ}}(w^n))\right| \leq \frac{MC_{T_1}C^{2}_{\ell}}{n^{2}\mu^{3}}, \quad \text{for } w^n \in \mathcal{D}^{-i}.
    \end{align}
\end{prop}

While certain loss functions may not be Lipschitz, \assref{ass:two_1} and \assref{ass:boundedmoments} require only that the {\em normalized} losses evaluated on the training set satisfy Lipschitz continuity— a condition that generally holds in practice \citep[Assump.~3]{giordano2019swiss}. Similarly, when the inference objective is of the form $\ell(z_{\mathrm{test}}, \theta)$, Lipschitz continuity is required only with respect to the test point $z_{\mathrm{test}}$. As long as $z_{\mathrm{test}}$ is not pathological, this assumption is typically satisfied.\footnote{The assumption that $T$ is Lipschitz is consistent with classical works on influence functions; see \citep[Prop.~1]{koh2019accuracy}.}

Additionally, the framework in \citep{giordano2019swiss} assumes differentiable regularization. In certain cases, similar approximations extend to settings where the regularizer is non-differentiable \citep{Wilson_OptimizerComparison, WilsonSuriyakumar_UnlearningProximal}.
   % While it is possible to construct examples where the loss function is not Lipschitz, \assref{ass:two_1} and \assref{ass:boundedmoments} only require that the normalized losses evaluated on the training set be Lipschitz -- a condition that typically holds in practice (see \citep[Assump.~3]{giordano2019swiss}). Similarly, when the inference objective takes the form $\ell(z_{\mathrm{test}}, \theta)$, Lipschitzness is required with respect to only a specific test point $z_{\mathrm{test}}$. Therefore, as long as $z_{\mathrm{test}}$ is not pathological, this Lipschitz assumption is generally satisfied.\footnote{The assumption that $T$ is Lipschitz is consistent with classical works on influence functions; see \citep[Prop.~1]{koh2019accuracy}.}

%We further note that the formulation from \citep{giordano2019swiss} considers cases where the regularization is differentiable. In some cases, similar approximations can be derived for the case where the regularizer is not differentiable (see \citep{Wilson_OptimizerComparison, WilsonSuriyakumar_UnlearningProximal}). 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{-4.5pt}
\subsection{Second-Order Approximations via the Natural Gradient}
\label{s:NGD}
% \vspace{-4.5pt}

This paper proposes a computationally efficient second-order approximation of $\hat{\theta}(w^{n})$ using the {\em natural gradient} to estimate influence. We consider loss functions $\ell$ that represent the log-likelihood of a parametric probabilistic model, where $P_{\sy|\sx}(y|x;\theta)$ lies on the probability simplex of the output alphabet $\pY$ and is parameterized by $\theta$ \citep{WhyNGD_Amari, Amari_InfoGeometry_Book}. While the standard gradient identifies the direction that minimizes the objective based on Euclidean distance, the natural gradient accounts for the underlying geometry (curvature) of the parameter space. This is achieved by pre-multiplying the gradient with the inverse of the Fisher Information Matrix (FIM), which characterizes the sensitivity of the model's likelihood function to changes in parameters.

A natural replacement for the Hessian in \eqref{eq:G_Definition} is the FIM \citep{NGD_Review}:
\begin{align}
    g_{Y|X} &\triangleq \nabla_{\theta} \log(P_{Y|X; \theta}(Y|X; \hat{\theta}(\boldsymbol{1}))),\\
    \brF(\hat{\theta}(\boldsymbol{1})) &\triangleq \mathbb{E}_{(X, Y) \sim P_{X,Y;\theta = \hat{\theta}(\boldsymbol{1})}}[ g_{Y|X} \cdot g_{Y|X}^\top ],
\end{align}
where $P_{Y|X}$ is the probabilistic model induced by the loss function. However, since the covariate distribution $P_{X}$ is typically unknown, direct computation of the expectation is infeasible. Instead, we approximate the FIM using empirical estimates, averaging over the observed covariates and leveraging the network structure to evaluate expectations over $P_{Y|X;\theta}$ \citep{NGD_Review, Limitations_FisherNGD}. The resulting \emph{approximate FIM} is given by:
\begin{align}
    \label{eq:Approx_FIM_Calc}
    \brF(\mD, \hat{\theta}(\boldsymbol{1})) \triangleq \frac{1}{n} \sum_{x \in \mD} \mathbb{E}_{Y \sim P_{Y|X=x;\theta=\hat{\theta}(\boldsymbol{1})}} [g_{Y|x} \cdot g_{Y|x}^\top ].
\end{align}
Using this approximation, we define the \emph{approximated Fisher infinitesimal jackknife} similarly to \eqref{eq:G_Definition}, replacing $\brC$ with the approximate FIM $\brF(\mD, \hat{\theta}(\boldsymbol{1}))$:
\begin{align}
    \label{eq:ApproximateFIM_Introduction}
     \tilde{\theta}^{\text{IJ,AF}}(w^{n}) \triangleq \hat{\theta}(\boldsymbol{1}) - (\brF(\mD,\hat{\theta}(\boldsymbol{1})))^{-1}b(\hat{\theta}(\boldsymbol{1}), w^{n}).
\end{align}


% This paper proposes using a computationally cheaper second-order approximation of $\hat{\theta}(w^{n})$ based on the {\em natural gradient} to calculate influence. We focus on loss functions $\ell$ that represent the log-likelihood of a parametric probabilistic model, where $P_{\sy|\sx}(y|x;\theta)$ lies on the probability simplex of the output alphabet $\pY$ and are controlled by the parameters $\theta$ \citep{WhyNGD_Amari, Amari_InfoGeometry_Book}. While the standard gradient is defined as the direction that minimizes the objective function based on Euclidean distance, the natural gradient incorporates the underlying geometry (curvature) of the parameter space, adjusting the gradient by pre-multiplying it with the inverse of the FIM. The FIM describes the shape of the likelihood surface, capturing the sensitivity of the model’s likelihood function to changes in the parameters.

% A starting option is to replace the Hessian in  \eqref{eq:G_Definition} with the following FIM \citep{NGD_Review}
% \begin{align}
%     % \label{eq:FisherInfo_Full}
%     g_{Y|X} &\defeq \nabla_{\theta} \log(P_{Y|X; \theta}(Y|X; \hat{\theta}(\boldsymbol{1}))),\\
%     \brF(\hat{\theta}(\boldsymbol{1})) &\defeq \mathbb{E}_{(X, Y) \sim P_{X,Y;\theta = \hat{\theta}(\boldsymbol{1})}}[ g_{Y|X} \cdot g_{Y|X}^\top ]
% \end{align}
% with $P_{Y|X}$ defined by the probabilistic model induced by the loss function. 
% However, the distribution of the covariates $P_{X}$ is not accessible, making this difficult to compute. We propose approximating the FIM using empirical estimates to average over the covariate samples and leverage the underlying network structure to evaluate the expectation over $P_{Y|X; \theta}$ \citep{NGD_Review, Limitations_FisherNGD}. This \emph{approximate FIM}, 
% is defined as 
% \begin{align}
%     \label{eq:Approx_FIM_Calc}
%     \brF(\mD, \hat{\theta}(\boldsymbol{1})) \defeq &\frac{1}{n}\sum_{x\in\mD}\mathbb{E}_{Y \sim P_{Y|X=x;\theta=\hat{\theta}(\boldsymbol{1})}} [g_{Y|x} \cdot g_{Y|x}^\top ].
% \end{align}
% With this approximation, we define the \emph{approximated Fisher infinitesimal jackknife} in a manner similar to \eqref{eq:G_Definition}, with $\brC$ replaced by the approximated FIM $\brF(\mD, \hat{\theta}(\boldsymbol{1}))$; namely, 
%  \begin{align}
%      % \label{eq:Fisher_Influence}
%      \tilde{\theta}^{\text{IJ,AF}}(w^{n}) \triangleq \hat{\theta}(\boldsymbol{1}) - (\brF(\mD,\hat{\theta}(\boldsymbol{1})))^{-1}b(\hat{\theta}(\boldsymbol{1}), w^{n}).\notag
%  \end{align}

% Finally, following classical developments (see, for example, \citep{Schraudolph_SecondOrder_VP} and \citep[Sec.~9.2]{NGD_Review}) when the loss function is given by  $\ell(z,\theta) = -\log(\CP{y}{f(x;\theta}))$ and $P(y|f)$ belongs to an exponential family, the approximated FIM can be viewed as a positive semi-definite (PSD) approximation of the Hessian. Specifically, the Hessian can be written as $\brH(\hat{\theta}(\boldsymbol{1}), \boldsymbol{1}) = \brF(\mD, \hat{\theta}(\boldsymbol{1})) + \brR$

% where $\brF(\mD, \hat{\theta}(\boldsymbol{1}))$ is guaranteed to be PSD and the matrix $\brR$ is given by 
% % \vspace{0pt}
% \begin{align}
%     \frac{1}{n}\sum^{n}_{i=1}\nabla^{2}_{\theta}f(x_i;\hat{\theta}(\boldsymbol{1}))\nabla_{f}\log(P(y_i|f(x_i;\hat{\theta}(\boldsymbol{1}))))
% \end{align}
% and is non-zero whenever the features are non-linear in the inputs. Furthermore,
% in many popular scenarios $\brR$ provably shrinks to zero (in the $L_2$ sense) as the model's \emph{training accuracy} improves (see \appref{app:exp_family_loss}, \appref{app:Prof_dist} and \citep{Limitations_FisherNGD, NGD_Review}). Thus, the approximated FIM is often interpreted as the PSD approximation of the Hessian. As we will prove in the subsequent sections, in many cases, similar guarantees can be obtained for $\tilde{\theta}^{\mathrm{IJ,AF}}(w^{n})$ and $\tilde{\theta}^{\mathrm{IJ}}(w^{n})$. However, since in many cases the natural gradient step is computationally cheaper than the Newton step, this approximation allows for a more efficient estimation of influence.


Following classical results \citep{Schraudolph_SecondOrder_VP, NGD_Review}, when the loss function is given by $\ell(z,\theta) = -\log(\CP{y}{f(x;\theta)})$ and $P(y|f)$ belongs to an exponential family, the approximate FIM can be interpreted as a positive semi-definite (PSD) approximation of the Hessian. Specifically, the Hessian satisfies:
\begin{align}
    \brH(\hat{\theta}(\boldsymbol{1}), \boldsymbol{1}) = \brF(\mD, \hat{\theta}(\boldsymbol{1})) + \brR,
\end{align}
where $\brF(\mD, \hat{\theta}(\boldsymbol{1}))$ is guaranteed to be PSD, and the remainder term is given by:
\begin{align}
    \frac{1}{n} \sum^{n}_{i=1} \nabla^{2}_{\theta} f(x_i;\hat{\theta}(\boldsymbol{1})) \nabla_{f} \log(P(y_i | f(x_i;\hat{\theta}(\boldsymbol{1})))).
\end{align}
This remainder term is nonzero whenever the features are non-linear in the inputs. However, in many settings, including commonly used models, $\brR$ shrinks to zero (in the $L_2$ sense) as training accuracy improves \citep{Limitations_FisherNGD, NGD_Review} (see \appref{app:exp_family_loss}, \appref{app:Prof_dist}). Thus, the approximated FIM is often viewed as a computationally efficient PSD approximation of the Hessian.

As we will demonstrate in the subsequent sections, similar guarantees can be established for $\tilde{\theta}^{\mathrm{IJ,AF}}(w^{n})$ and $\tilde{\theta}^{\mathrm{IJ}}(w^{n})$. However, since natural gradient updates are often computationally cheaper than Newton steps, this approximation enables more efficient influence estimation.

==> computation.tex <==
\section{Computational Savings}
\label{s:CompCost}
% \vspace{-4.5pt}
Here, we show a fundamental efficiency improvement in evaluating \eqref{eq:Distance_Approx_eq} compared to the IJ approach. Both methods require computing expressions of the form $\brA^{-1}b(\hat{\theta}(\boldsymbol{1}), w^{n})$ where $\brA = \brF(\mD, \hat{\theta}(\boldsymbol{1}))$ in \eqref{eq:Distance_Approx_eq} and $\brA = \brH(\hat{\theta}(\boldsymbol{1}), \boldsymbol{1})$ for the IJ\ \footnote{Adding a regularization term to these matrices negligibly affects computational complexity.}. Since directly inverting a large $d \times d$ matrix is infeasible, efficient computation of inverse-matrix-vector products is essential.
Following \citep{KohLiang_Influence_DL}, the dominant method for these calculations is stochastic estimation using the \texttt{LiSSA} algorithm \citep{HazanAgrawal_Lissa}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{-4.5pt}
\subsection{Stochastic Estimation}
\label{s:Stochastic_Lissa}
% \vspace{-4.5pt}
Let $v_j \triangleq (\widehat{\brA^{-1}x})_j$. Every influence assessment technique discussed so far generates estimators $v_j$ that converge in expectation to $\brA^{-1}x$ as $j \to \infty$, each utilizing small batches of training data. The \texttt{LiSSA} algorithm approximates $\brA^{-1}$ using the truncated Neumann series $\brA^{-1}_j = \sum_{i=0}^{j} (\brI - \sigma\brA)^i$ for some $\sigma > 0$\ \footnote{$\sigma$ is usually a small positive constant to stabilize calculations.}. This approximation is computed via the recursion $\brA^{-1}_j = \brI + (\brI - \sigma\brA)\brA^{-1}_{j-1}$. Consequently, each $v_j$ is defined by $v_j = x + (\brI - \sigma\brA)v_{j-1}$
with $v_0 = x$ and final estimate $v = \sigma v_N$. The major computational hurdle is multiplying by $\brA$. When $\brA$ depends on many training points (e.g., $\brF(\mD, \hat{\theta}(\boldsymbol{1}))$ or $\brH(\hat{\theta}(\boldsymbol{1}), \boldsymbol{1})$), it is typical to estimate it by using a sampled batch of training data. We now analyze the computational complexity of these calculations for each method. 

% \vspace{-4.5pt}
\paragraph{Estimation with $\brF(\mD, \hat{\theta}(\boldsymbol{1}))$.}
\label{s:Stochastic_FIM}
% \vspace{-4.5pt}
When $\brA \defeq \brF(\mD, \theta)$, each $\brA v_j$ requires calculating
\begin{align} 
    \label{eq:Esimtates_FIM}
    &\nabla_{\theta} f_i \cdot (\nabla^{2}_{f} \log( \CP{y_i}{f_i}) )(v^{\top}_j\nabla_{\theta} f_i)^{\top})
\end{align}
where $f_i \triangleq f(x_i;\theta)$. Given the form of $\nabla^{2}_{f} \log(\CP{y_j}{f(x_j; \theta)})$ (see \appref{app:exp_family_loss}), computing this expression requires the vector-Jacobian product (VJP) $a_j = v^{\top}_j\nabla_{\theta} f_i$ and the Jacobian-vector product (JVP) $\nabla_{\theta} f_i \cdot (\nabla^{2}_{f} \log( \CP{y_i}{f_i}) )a^{\top}_j)$.

% \vspace{-6pt}
\paragraph{Estimation with $\brH(\hat{\theta}(\boldsymbol{1}), \boldsymbol{1})$.}
% \vspace{-4.5pt}
\label{s:Stochastic_Hessian}
For $\brA \defeq \brH(\hat{\theta}(\boldsymbol{1}),\boldsymbol{1})$, each $\brA v_j$ requires computing,
% \vspace{-\baselineskip}
\begin{align}
    \label{eq:Stochastic_Hess}
    \nabla^{2}_{\theta}\log(\CP{y_i}{f_i})v_j, 
\end{align}
% \vspace{-\baselineskip}
which requires computing a Hessian-vector product (HVP) with respect to all model parameters.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{-12pt}
\paragraph{Comparing Computations.}
% \vspace{-4.5pt}
Computing \eqref{eq:Stochastic_Hess} requires roughly four evaluations of the entire model \citep{Schraudolph_SecondOrder_VP, iclr2024_hvp}. In contrast, a JVP can be computed in a single forward pass using forward-mode automatic differentiation \citep{JAX_autodiff_cookbook}. Since $\nabla^{2}_{f}\log(\CP{y_i}{f_i})$ is typically simple and depends only on the number of model outputs (not on $d$), evaluating \eqref{eq:Esimtates_FIM} requires just one differentiation in backward mode. Furthermore, given backward differentiation roughly requires twice the complexity of model evaluation \citep{deepspeed_flops, iclr2024_hvp}, this method significantly reduces FLOPs and accelerates computations. We demonstrate these savings through simulations in \secref{s:Exps}. We summarize the results in \tblref{tbl:passes}. 

\setlength{\tabcolsep}{4pt} 
\begin{table}[h!]
\centering
\begin{tabular}{lccc}
\toprule
\textbf{} & \textbf{\shortstack{Forward}} & \textbf{\shortstack{Backward}} & \textbf{FLOPs} \\
\midrule
\eqref{eq:Stochastic_Hess}      & 0   & 2     & $O(4F)$ \\
\eqref{eq:Stochastic_Hess}      & 2   & 1     & $O(4F)$ \\
\eqref{eq:Esimtates_FIM}        & 1   & 1     & $O(3F)$  \\
\bottomrule
\end{tabular}
\caption{Number of differentiations in forward mode, backward mode, and FLOPs required to evaluate \eqref{eq:Esimtates_FIM} and \eqref{eq:Stochastic_Hess}, for different evaluation options from \citep{iclr2024_hvp}. $F$ denotes the FLOPs needed for a single model evaluation.}
\label{tbl:passes}
\end{table}

==> our_method.tex <==
\section{Main Result}
\label{s:MainResult}
% \vspace{-4.5pt}
We now present a theoretical characterization of the performance of the approximate Fisher influence, based on the approximation defined in \eqref{eq:ApproximateFIM_Introduction}. First, we introduce a set of technical assumptions, which are essential for our proofs.
\begin{assump}
    \label{ass:LossFunc_ExpFamily}
    The loss functions are of the form $\ell(z, \theta) = -\log(\CP{y}{f(x;\theta)})$ where $\CP{y}{f}$ belongs to an exponential family whose natural parameters are $f(x;\theta)$. Moreover, we further assume that $-\nabla^{2}_{f}\log\left(\CP{y}{f(x;\theta)}\right) \preceq Q\cdot\brI_d$ \ for some $Q > 0$.
\end{assump}

To accommodate non-smooth regularizers, we utilize the \emph{proximal operator}, defined as:
% \vspace{-2pt}
\begin{align}
    \text{prox}^{\brD}_{\lambda \pi}(v) \triangleq \underset{\theta}{\argmin} \ \left\{(v - \theta)^{\top}\brD(v - \theta) + 2\lambda \pi(\theta)\right\}.\notag
\end{align}
%\vspace{-4.5pt}
Our main lemma, \lemref{lem:Distance}, defines the approximate Fisher influence and bounds its discrepancy from $\hat{\theta}(w^n)$ for $w^n \in \mathcal{D}^{-i}$.

\begin{lem}
\label{lem:Distance}
Suppose \assref{ass:one_1}, \assref{ass:two_1}, \assref{ass:LipFeatures}, and \assref{ass:LossFunc_ExpFamily} hold. Define
$\bar{E}_n \triangleq \sum^{n}_{j=1}\|\nabla_{f}\log(P(y_j|f(x_j;\hat{\theta}(\boldsymbol{1}))))\|$, $\tilde{g}_{i} \triangleq \|\nabla_{\theta}\ell(z_i, \hat{\theta}(\boldsymbol{1}))\|$ and $g_i = \tilde{g}_i/n$. Then, the approximated Fisher influence satisfies
\begin{align}
    \label{eq:Distance_Approx_eq} 
    \tilde{\theta}(w^n) &= \mathrm{Prox}^{\brF(\mD, \hat{\theta}(\boldsymbol{1}))}_{\lambda\pi}(\tilde{\theta}^{\mathrm{IJ,AF}}(w^n)), \quad \text{for } w^n \in \mathcal{D}^{-i}.
\end{align}
Furthermore, the discrepancy between $\tilde{\theta}(w^n)$ and $\hat{\theta}(w^n)$ is bounded as:
\begin{align}
    \label{eq:DistBound_Lem}
    \|\tilde{\theta}(w^n) - \hat{\theta}(w^n)\| \leq \frac{2Q C^{2}_f \tilde{g}_{i}}{n^{2}\mu^{2}} + \frac{M\tilde{g}_{i}^{2}}{n^2\mu^3} + \frac{2\tilde{g}_i\tilde{C}_f\bar{E}_n}{n\mu^{2}}, \quad \text{for } w^n \in \mathcal{D}^{-i}.
\end{align}
\end{lem}
% \vspace{-3pt}
% Our main lemma, \lemref{lem:Distance}, defines our approximation and bounds its discrepancy from $\hat{\theta}(\boldsymbol{1}^{n\backslash i})$:
% \begin{lem}
% \label{lem:Distance}
% Suppose \assref{ass:one_1}, \ref{ass:two_1}, 
% \ref{ass:LipFeatures} and \ref{ass:LossFunc_ExpFamily} hold. Let $\bar{E}_n \triangleq \sum^{n}_{j=1}\|\nabla_{f}\log(P(y_j|f(x_j;\hat{\theta}(\boldsymbol{1}))))\|$, $\tilde{g}_{i} \triangleq \|\nabla_{\theta}\ell(z_i, \hat{\theta}(\boldsymbol{1}))\|$ and $g_i = \tilde{g}_i/n$. Then 
%     \begin{align}
%          \label{eq:Distance_Approx_eq} 
%         \tilde{\theta}(\boldsymbol{1}^{n\backslash i}) &= \mathrm{Prox}^{\brF(\mD, \hat{\theta}(\boldsymbol{1}))}_{\lambda\pi}(\tilde{\theta}^{\mathrm{IJ,AF}}(\boldsymbol{1}^{n\backslash i}))
%     \end{align}
%     satisfies  
%     \begin{align}
%         \label{eq:DistBound_Lem}
%         \|\tilde{\theta}(\boldsymbol{1}^{n\backslash i}) - \hat{\theta}(\boldsymbol{1}^{n\backslash i})\| \leq \frac{2Q C^{2}_f \tilde{g}_{i}}{n^{2}\mu^{2}} + \frac{M\tilde{g}_{i}^{2}}{n^2\mu^3} + \frac{2\tilde{g}_i\tilde{C}_f\bar{E}_n}{n\mu^{2}}.
%     \end{align}
% \end{lem}
\noindent {\em Proof sketch.}
The proof separately bounds the distances between (i) $\hat{\theta}(w^n)$ and $\tilde{\theta}^{\text{IJ}}(w^n)$, and (ii) $\tilde{\theta}^{\text{IJ}}(w^n)$ and $\tilde{\theta}^{\mathrm{IJ,AF}}(w^n)$ for $w^n \in \mathcal{D}^{-i}$. The first bound follows from \citep[Lem.~1]{Wilson_OptimizerComparison}, while the second leverages the smoothness properties of the function to show that the estimates remain close.  
   % The proof treats the distance between $\hat{\theta}(\boldsymbol{1}^{n\backslash i})$ to $\tilde{\theta}^{\text{IJ}}(\boldsymbol{1}^{n\backslash i})$ and $\tilde{\theta}^{\text{IJ}}(\boldsymbol{1}^{n\backslash i})$ to $\tilde{\theta}^{\mathrm{IJ,AF}}(\boldsymbol{1}^{n\backslash i})$ separately. The first bound is proved in \citep[Lem.~1]{Wilson_OptimizerComparison}, and the second makes use of the smoothness properties of the function to conclude the estimates are close. 
\qed

The full proof is provided in \appref{app:Prof_dist}. Similar to prior results \citep{Wilson_OptimizerComparison, WilsonSuriyakumar_UnlearningProximal, Sekhari_Unlearning_Neurips}, the first two terms in \eqref{eq:DistBound_Lem} depend on global problem constants (Lipschitz coefficients, strong convexity parameter, etc.) and the gradient at the $i$th training point. The third term depends on $\bar{E}_n$, which simplifies due to the exponential family structure of the loss:
\begin{align}
    \|\nabla_{f}\log(P(y_i|f(x_i;\hat{\theta}(\boldsymbol{1}))))\| = \|t(y_i) - \Esub{\sy\sim P_{Y|X = x_i;\hat{\theta}(\boldsymbol{1})}}{t(Y)}\|.
\end{align}
Thus, $\bar{E}_n$ serves as an upper bound on the gradient at the optimum $\hat{\theta}(\boldsymbol{1})$ (see \appref{app:exp_family_loss}, \appref{s:Loss_ExpFamily}). In \appref{app:exp_family_loss}, we further demonstrate how this term relates to the absolute training error in classification and regression problems. Specifically, as training error decreases, this term also diminishes. In the extreme case where $\ell(z_i, \hat{\theta}(\boldsymbol{1})) = 0$ for all $i \in [n]$, this term is exactly zero; we provide details in \appref{app:Prof_dist}.  
For the remaining terms in \lemref{lem:Distance}, the worst-case discrepancy between $\tilde{\theta}(w^n)$ and $\hat{\theta}(w^n)$ for all $i \in [n]$ is controlled by $
g_{\max} \triangleq \max_{i\in[n]} g_{i}.$
By \assref{ass:boundedmoments} with $(s, r) = (0,1)$, $g_{\max}$ is finite.  

Next, we present our main theorem, which establishes error bounds for the approximated inference objective $T(\cdot)$.

% Full proof details are contained in \appref{app:Prof_dist}. Similar to the bound presented in previous works \citep{Wilson_OptimizerComparison, WilsonSuriyakumar_UnlearningProximal, Sekhari_Unlearning_Neurips}, the first two terms in \eqref{eq:DistBound_Lem} depend on global problem constants (Lipschitz coefficients, strong convexity parameter, \etc) and the gradient on the $i$'th training point. The third term depends on $\bar{E}_n$; in particular, the exponential family structure of the loss leads to the simplification $\|\nabla_{f}\log(P(y_i|f(x_i;\hat{\theta}(\boldsymbol{1}))))\| = \|t(y_i) - \Esub{\sy\sim P_{\sy|\sx = x_i;\hat{\theta}(\boldsymbol{1})}}{t(\sy)}\|$. Thus, $\bar{E}_n$ corresponds to an upper bound on the gradient at the optimum $\hat{\theta}(\boldsymbol{1})$ (see \appref{app:exp_family_loss}, \appref{s:Loss_ExpFamily}). In \appref{app:exp_family_loss} we further show how this term relates to the training error's absolute value in classification and regression problems and show how this term gets smaller whenever the train error decreases. In the extreme case where $\ell(z_i, \hat{\theta}(\boldsymbol{1})) = 0, \forall i\in[n]$ this term is exactly $0$, and we provide details for this fact in \appref{app:Prof_dist}. For the other terms in \lemref{lem:Distance}, we see that the worst case discrepancy between $\tilde{\theta}(\boldsymbol{1}^{n\backslash i})$ and $\hat{\theta}(\boldsymbol{1}^{n\backslash i}), \forall i\in [n]$ depends on how small $g_{\max}$ is where $g_{\max} \triangleq \max_{i\in[n]} g_{i}$. \assref{ass:boundedmoments} with $(s, r) = (0, 1)$ requires $g_{\max}$ is finite. Next, we prove our main theorem that provides error bounds on the approximated $T(\cdot)$. 

\begin{thm}
    \label{thm:objective_bound}
    Suppose \assref{ass:one_1}, \assref{ass:two_1}, and \assref{ass:LipFeatures}-\assref{ass:LossFunc_ExpFamily} hold. 
    Let $\tilde{\theta}(w^n)$ be defined as in \eqref{eq:Distance_Approx_eq} for $w^n \in \mathcal{D}^{-i}$. Then, 
    \begin{align}
        \label{eq:Objective_bound_final}
        \|T(\hat{\theta}(w^n)) - T(\tilde{\theta}(w^n))\| 
        &\leq C_{T_1} \left( \frac{2Q C^{2}_f \tilde{g}_{i}}{n^{2}\mu^{2}} + \frac{M\tilde{g}_{i}^{2}}{n^{2}\mu^3} + \frac{2\tilde{g}_i\tilde{C}_f\bar{E}_n}{n\mu^{2}} \right) \\
        &\quad + \frac{1}{2} C_{T_2} \left( \frac{2Q C^{2}_f \tilde{g}_{i}}{n^{2}\mu^{2}} + \frac{M\tilde{g}_{i}^{2}}{n^{2}\mu^3} + \frac{2\tilde{g}_i\tilde{C}_f\bar{E}_n}{n\mu^{2}} \right)^{2}.
    \end{align}
    Moreover, 
    \begin{align}
        \label{eq:Taylor_Proof}
        \| T(\hat{\theta}(w^n)) &- T(\hat{\theta}(\boldsymbol{1})) 
        - \langle \nabla T(\hat{\theta}(\boldsymbol{1})), \tilde{\theta}(w^n) - \hat{\theta}(\boldsymbol{1}) \rangle \| \\
        &\leq C_{T_1} \left( \frac{2Q C^{2}_f \tilde{g}_{i}}{n^{2}\mu^{2}} + \frac{M\tilde{g}_{i}^{2}}{n^{2}\mu^3} + \frac{2\tilde{g}_i\tilde{C}_f\bar{E}_n}{n\mu^{2}} \right) + \frac{2C_{T_2}\tilde{g}^{2}_i}{n^{2}\mu^{2}}.
    \end{align}
\end{thm}
\noindent {\em Proof sketch.}
    % Both bounds crucially rely on smoothness properties of $T$ (\assref{ass:Lipschitz_T}) in combination with \lemref{lem:Distance} and \lemref{lem:gen_strong_convex} from \appref{app:Closeness_Weighted}.  \qed
    Both bounds follow from the smoothness properties of \( T \) (\assref{ass:Lipschitz_T}), combined with \lemref{lem:Distance} and \lemref{lem:gen_strong_convex} from \appref{app:Closeness_Weighted}.  \qed
%\end{proof}

Full proof details are provided in \appref{app:InferenceObjective_Bound}. \thmref{thm:objective_bound} enables a systematic derivation of theoretical guarantees for FIM-based influence approximations across various application areas, categorized into the following three settings.

As discussed in \citep[Sec.~3]{giordano2019swiss}, for weight vectors \( w^n = \mathcal{D}^{-i} \), we expect \( \lim_{n\to\infty} g_{\max} = 0 \). Consequently, whenever \( \bar{E}_n \to 0 \), \thmref{thm:objective_bound} ensures that \( T(\tilde{\theta}(w^n)) \) and the Taylor-series approximation (Equation~\eqref{eq:TaylorSeries_Objective} with \( w^n \in \mathcal{D}^{-i} \)) converge to \( T(\hat{\theta}(w^n)) \) for all \( i \in [n] \).

However, as we demonstrate in \secref{s:Exp_Fairness} and \secref{s:Exp_CV}, in practice, \( \tilde{\theta}(w^n) \) is often a good approximation of \( \hat{\theta}(w^n) \) even when \( \bar{E}_n \) is finite.

%  Full proof details are contained in~\appref{app:InferenceObjective_Bound}. \thmref{thm:objective_bound} allows us to systematically obtain theoretical guarantees for FIM-based approximations of influence across several application areas, illustrated in the following three categories. 
% As discussed in \citep[Sec.~3]{giordano2019swiss}, for vectors $w^n = \boldsymbol{1}^{n\backslash i}$, we expect $\lim_{n\to\infty} g_{\max} = 0 $. Consequently, whenever $\bar{E}_n \to 0$ \thmref{thm:objective_bound} shows that $T(\tilde{\theta}(\boldsymbol{1}^{n\backslash i}))$ and the Taylor-series approximation (\eqref{eq:TaylorSeries_Objective} with $w^{n} = \boldsymbol{1}^{n\backslash i}$) converges to $T(\hat{\theta}(\boldsymbol{1}^{n\backslash i})), \forall i\in[n]$. 
% However, as we will show in \secref{s:Exp_Fairness} and \secref{s:Exp_CV}, in practice, $\tilde{\theta}(\boldsymbol{1}^{n\backslash i})$ {\em is often a good approximation to $\hat{\theta}(\boldsymbol{1}^{n\backslash i})$, even when $\bar{E}_n$  is finite}. 

% Next, we demonstrate that our framework offers guarantees in a unified way parallel to \propref{prop:CV_Guarantees_Wilson} - \propref{prop:attributions}, which use Hessian-based methods for several tasks outlined in \secref{s:ProblemDef}. 
Next, we show that our framework provides guarantees in a unified manner, analogous to \propref{prop:CV_Guarantees_Wilson}–\propref{prop:attributions}, which establish Hessian-based guarantees for several tasks outlined in \secref{s:ProblemDef}.

\begin{corol}[LOOCV]
\label{corol:LOOCV_FIM}
Suppose \assref{ass:one_1}, \assref{ass:two_1}, and \assref{ass:boundedmoments}-\assref{ass:LossFunc_ExpFamily} hold with $(s,r) = \{(0, 2), (0, 3), (1, 2), (1, 3), (1, 4)\}$. Let \( T_i(\theta) = \frac{1}{n} \ell(z_i, \theta) \). When \( \tilde{\theta}(w^n) \) from \lemref{lem:Distance} is used as a plug-in estimate for \( w^n \in \mathcal{D}^{-i} \), the error in the approximate cross-validation estimate satisfies:
\begin{align}
    \left| \sum_{i=1}^n \left( T_i(\tilde{\theta}(w^n)) - T_i(\hat{\theta}(w^n)) \right) \right| 
    \leq O\left( \frac{MB_{03}}{\mu^3 n^2} + \frac{C^{2}_f B_{02}}{\mu^{2} n^{2}} + \frac{\tilde{C}_f \bar{E}_n B_{02}}{\mu^{2} n} \right).
\end{align}
\end{corol}

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{corol}[Machine Unlearning]
\label{corol:unlearning_FIM}
Suppose \assref{ass:one_1}, \assref{ass:two_1}, \assref{ass:LipFeatures}, and \assref{ass:LossFunc_ExpFamily} hold. Assume further that \( \tilde{g}_i \leq G \) for all \( i \in [n] \). Then, for the inference objective \( T(\theta) = \theta \), we have:
\begin{align}
    \|T(\tilde{\theta}(w^n)) - T(\hat{\theta}(w^n))\| 
    \leq \frac{2Q C^{2}_f G}{n^{2}\mu^{2}} + \frac{MG^{2}}{n^{2}\mu^3} + \frac{2G\tilde{C}_f\bar{E}_n}{n\mu^{2}}, \quad \text{for } w^n \in \mathcal{D}^{-i}.
\end{align}
Furthermore, the algorithm returning \( \tilde{\theta}(w^n) + \zeta \) satisfies \( (\eps, \delta) \)-unlearning, where \( \zeta \sim \mathcal{N}(0 ,c\brI) \) and:
\begin{align}
    c = \left( \frac{2Q C^{2}_f G}{n^{2}\mu^{2}} + \frac{MG^{2}}{n^{2}\mu^3} + \frac{2G\tilde{C}_f\bar{E}_n}{n\mu^2} \right) \frac{\sqrt{2\log(5/4\delta)}}{\eps}.
\end{align}
\end{corol}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{corol}[Data Attribution] 
\label{corol:Attributed_FIM}
    Suppose the assumptions of \thmref{thm:objective_bound} hold, $T(\theta) = \ell(z_{\mathrm{test}}, \theta) - \ell(z_{\mathrm{test}}, \hat\theta(\boldsymbol{1}))$ and $C_{\ell} \triangleq \underset{i\in[n]}{\max} \ \tilde{g}_i$. Then,  
    % \vspace{-8pt}
    \begin{align}
        &|T(\hat{\theta}(\boldsymbol{1}^{n\backslash i})) - T(\tilde{\theta}(\boldsymbol{1}^{n\backslash i}))| \leq O(\frac{C^2_f C_{T_1}C_{\ell}}{n^2\mu^2} + \frac{M C_{T_1}C^{2}_{\ell}}{n^2\mu^3} + \frac{C_{T_1}\tilde{C}_f\bar{E}_nC_{\ell}}{n\mu^2}), \\ 
           &| T(\hat{\theta}(\boldsymbol{1}^{n\backslash i})) - T(\hat{\theta}(\boldsymbol{1})) - \langle \nabla T(\hat{\theta}(\boldsymbol{1})),\tilde{\theta}(\boldsymbol{1}^{n\backslash i}) -\hat{\theta}(\boldsymbol{1})\rangle | \notag\\ 
         &\qquad\qquad \leq O(\frac{C^2_f C_{T_1}C_{\ell}}{n^2\mu^2}  + \frac{M C_{T_1}C^{2}_{\ell}}{n^2\mu^3}  + \frac{C_{T_2}C^{2}_{\ell}}{n^2\mu^2}  + \frac{C_{T_1}\tilde{C}_f\bar{E}_nC_{\ell}}{n\mu^2})
    \end{align}
\end{corol}

The proofs for these corollaries rely on applying \thmref{thm:objective_bound} for the settings described in \propref{prop:CV_Guarantees_Wilson} - \propref{prop:attributions} (see \appref{app:corol_proofs}). To further demonstrate the generality of our approach, we provide guarantees for the fairness assessment task described in \secref{s:ProblemDef}, for which currently there is no theoretical analysis. The proof is in \appref{app:corol_Fairness}. 
\begin{corol}[Fairness Assessments]
    \label{corol:fairness}
    Suppose \assref{ass:one_1}, \assref{ass:two_1}, and \assref{ass:LipFeatures} -\assref{ass:LossFunc_ExpFamily} hold. If $T$ be given by \eqref{eq:DP_Def} and $C_{\ell} \triangleq \underset{i\in[n]}{\max} \ \tilde{g}_i$. Then, 
    \vspace{0pt}
    \begin{align}
        &|T(\hat{\theta}(\boldsymbol{1}^{n\backslash i})) - T(\tilde{\theta}(\boldsymbol{1}^{n\backslash i}))| \leq O(\frac{C^3_fC_{\ell}}{n^2\mu^2} + \frac{M C_fC^{2}_{\ell}}{n^2\mu^3} + \frac{C_f\tilde{C}_fC_{\ell}\bar{E}_n}{n\mu^2}).
    \end{align}
\end{corol}
To the best of our knowledge, \corolref{corol:LOOCV_FIM} - \corolref{corol:fairness} provide the first theoretical guarantees for using the FIM in influence assessment tasks, offering a novel method with rigorous effectiveness proof. Additionally, our framework easily extends to other problems in machine learning and statistics beyond the specific applications discussed (e.g., data dropping \citep{Broderick_Robustness}). 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{-4.5pt}
\subsection{The Non-Convex Setting}
\label{s:NonConvex}
% \vspace{-4.5pt}
While, like many theoretical analyses of influence (e.g. \citep{KohLiang_Influence_DL}) our theory assumes a convex, differentiable loss, this assumption does not hold in many practical scenarios. Nonetheless, influence functions are still widely used for influence assessment \citep{KohLiang_Influence_DL, han2020explaining}. Recent work by \citep{Bae_PBRF_Influence} 
show that a variant of Fisher influence corresponds to the minimizer of an approximation to the Proximal Bregman Response Function (PBRF), which helps to explain the empirical utility of influence functions in complex domains. Our probabilistic framework extends these results by introducing $\tilde{\theta}(\boldsymbol{1}^{n\backslash i})$ that depends on $\tilde{\theta}^{\mathrm{IJ,AF}}(\boldsymbol{1}^{n\backslash i})$ and can be efficiently computed. Moreover, our framework allows us to theoretically justify the usage of the AFIF and to further bound the distance $\|\tilde{\theta}^{\text{IJ}}(\boldsymbol{1}^{n\backslash i}) - \tilde{\theta}(\boldsymbol{1}^{n\backslash i})\|$ under mild assumptions that are likely to hold locally (see \appref{app:dist_bound_IJ_F}). This supports the use of AFIF over traditional Hessian-based methods. Moreover, while \citep{Bae_PBRF_Influence} focuses on $\pi(\theta) = \norm{\theta}^2$, our framework easily accommodates non-differentiable regularizers.

\noindent {\em Remark on the computational stability.}
%    \label{rem:Stability}
    Both \eqref{eq:G_Definition} and \eqref{eq:Distance_Approx_eq} require their respective matrices, $\brH(\hat{\theta}(\boldsymbol{1}), \boldsymbol{1})$ and $\brF(\mD, \hat{\theta}(\boldsymbol{1}))$, be invertible. $\brF(\mD, \hat{\theta}(\boldsymbol{1}))$ is PSD, so adding a small regularization term $\epsilon \brI$ (with $\epsilon > 0$) ensures invertibility. However, since $\brH(\hat{\theta}(\boldsymbol{1}), \boldsymbol{1})$ may not be PSD in the non-convex setting, regularizing \eqref{eq:G_Definition} generally requires extra hyperparameter tuning and can introduce instabilities. This is an additional advantage of using the AFIF when the loss is non-convex.
%\end{remark}
